Two of a Kind: Comparing big and small black holes in binaries with gravitational waves

When modeling the population of merging binary black holes, analyses have generally focused on characterizing the distribution of primary (i.e. more massive) black holes in the binary, while simplistic prescriptions are used for the distribution of secondary masses. However, the secondary mass distribution and its relationship to the primary mass distribution provide a fundamental observational constraint on the formation history of coalescing binary black holes. If both black holes experience similar stellar evolutionary processes prior to collapse, as might be expected in dynamical formation channels, the primary and secondary mass distributions would show similar features. If they follow distinct evolutionary pathways (for example, due to binary interactions that break symmetry between the initially more massive and less massive star), their mass distributions may differ. We present the first analysis of the binary black hole population that explicitly fits for the secondary mass distribution. We find that the data is consistent with a $\sim30\,M_{\odot}$ peak existing only in the distribution of \emph{secondary} rather than primary masses. This would have major implications for our understanding of the formation of these binaries. Alternatively, the data is consistent with the peak existing in both component mass distributions, a possibility not included in most other previous studies. In either case, the peak is observed at $31.4_{-2.6}^{+2.3}\,M_{\odot}$, which is shifted lower than the value obtained in previous analyses of the marginal primary mass distribution, placing this feature in further tension with expectations from a pulsational pair-instability supernova pileup.

==> old.tex <==
% old text that I couldn't bring myself to delete/may need later

\begin{figure*}
    \centering
    \includegraphics{figures/p_m2_paper_flow.pdf}
    \caption{Outline for the paper, given a few possible results. Numbers correspond to the main questions we want to answer.
    How we will answer them is addressed in Figure~\ref{fig:methods}}
    \label{fig:outline}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics{figures/p_m2_paper_methods.pdf}
    \caption{How we will answer the questions enumerated in Figure~\ref{fig:outline}}*
    \label{fig:methods}
\end{figure*}


\subsection{Primary and Secondary Masses are consistent with being drawn from the same underlying distribution}
\label{sec:diff vs same}

Once we fit the \comment{insert nickname here} model, we compare the inferred hyperparameters of both the primary and secondary mass distributions ($\Lambda_1$ and $\Lambda_2$, respectively) and determine whether they are consistent.

\begin{enumerate}
    \item summary of section: To determine if  primary and secondary masses are drawn from the same distribtuion (subject to a pairing function) we fit a model in which the two distributions are allowed to be separate, compare the inferred hyperparameters of both the primary and secondary mass distributions ($\Lambda_1$ and $\Lambda_2$, respectively), and determine whether they are consistent with one another.
    We then asses the performance of this model compared to one in which the two distrbutions are forced to be described by the same exact hyperparameters (i.e. $\Lambda_1 = \Lambda_2$).
    Finally, we focus on the peak previously found in the primary mass distribution at $\sim35\Msun$ using the pairing function formalism and determine if it exists in the primary mass distribution, the secondary mass distribution, or both.
    \item To determine the consistency of $p(m_1)$ with $p(m_2)$, we first directly compare the posteriors of hyperparameters $\Lambda_1$ and $\Lambda_2$. 
    We then create a model in which we impose $\Lambda_1 = \Lambda_2$ and compare the performance of that model to the one in which $\Lambda_1$ does not necessarily equal $\Lambda_2$.
    \comment{We don't really do this, but we do compare $\lambda_1$ and $\lambda_2$}
    \item We perform PPCs \comment{insert and describe quantitative results} and find that both models perform equally well: we cannot tell if the two distributions are different, but since one is a subset of the other and the subset doesn't perform worse, its plausible that they could be the same. 
    We therefore use the p(m) model for the rest of the paper.
\end{enumerate}


\subsection{The secondary mass distribution exhibits an overdensity at $m_2\sim35\Msun$}
\begin{itemize}
    \item The bump at $\sim35\Msun$ has garnered significant interest, but under the fiducial pl+p model, it is unclear whether it only exists in one of the component masses or both. It is modeled as a feature in the primary mass distribution, but it is plausible that the secondary masses are actually driving the existence of the feature.  With our pairing function model we can being to figure out which component the feature is in.
    \item one of the lambdas can be zero but not both: plot of lambda1 lambda2 posteriors, along with their marginals
    \item Unclear if its because m2 has its own bump or because m1 has a bump and we prefer equal masses (how are these actually different? they both lead to similar marginal m2s, right? but i guess they lead to different conditional m2s, which means they are different)
    \item To test this, we run a variant of the usual model where we set $\lambda_2=0$ and tried to see if it underpredicted the number of events in the $\sim35\Msun$ region (a PPC). 
    \item It doesn't, but the usual model doesn't overpredict events in that region, so right now we can't tell.
    \item this is partially because we can still generate an overdensity of events wit hm2 in that peak just by having a picker pairing function. Indeed, betaq is larger under the lambda2=0 model. 
    \item In future observing runs, we will be able to tell these two scenarios apart by ...
    \item Seems like m2 is driving the bump. lam2!=0 and lam1 is consistent with zero when we fix all other parameters between the two models. 
    Again, we can't tell if m1 actually doesn't want a bump bc the m1s will have a bump if m2 has a bump bc BBHs are picky. 
    Conditional distribution of m1 given m2 looks identical between all power law pairing function models.
\end{itemize}

\subsection{Data prefer a model with $\Lambda_1=/\neq \Lambda_2$}
\begin{itemize}
    \item p(m) performs better/worse/the same on a PPC and with BFs than using different p1 and p2
    \item since they are the same, we can use p(m) for the rest of the paper
\end{itemize}

\subsection{Model selection}
\label{sec:model selection}
\comment{can probably remove this section.}
\mayac{Agree. I think the later statements about how future data will tell apart the models are sufficient.}
We perform several posterior predictive checks (PPCs) on the models considered in this work and find that with the current number of detections, we are unable to determine which model is preferred by the data. 

In Figure~\ref{fig:PPCs}, we plot the posterior predictive distributions of detected secondary masses, conditioned on $m_1=35\Msun$ and $m_1>50\Msun$ for the \qdist{} and \default{} models.
We also show the observed data under each of these models and conditioned on the same values of $m_1$.

Both models show general agreement between predictions and observations.
The largest discrepancy in predicted populations between the two models occurs in the regions $m_1\in[30,40] \cap m_2\in[m_{\min},30]$, so comparing the number of detected versus predicted events in that region is the most sensitive metric to select between the models.
\qdist{} predicts \result{X} detections with $m_1\in[30,40]$ and $m_2\in[m_{\min},30]$, and \result{Y} events are observed in that region.
\default{} predicts \result{X} events and observes \result{Y} events in that same region.
Differences in the number of observed events between the two models is due to event-level parameter uncertainty: the event component mass posteriors change depending on the population prior since the likelihoods are broad.

Because of the large uncertainties in these PPCs, we are unable to determine which model provides a more accurate description of the data and conclude that both formalisms are consistent with current observations.

\comment{Could put predictions here if we remove the ``implications'' sections}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/PPCs.pdf}
    \caption{Secondary mass posterior predictive distributions conditioned on $m_1=35\Msun$ (\emph{top}) and $m_1>50\Msun$ (\emph{bottom}) for the \qdist{} and \default{} models.
    In contrast to Figure~\ref{fig:conditional ppds}, this shows the \emph{detected} distribution of sources.
    Solid lines indicate predictions, where dashed lines indicate observations. Both models show consistency between predictions and observations, though posterior predictive checks are known to be less sensitive when performed on event-level parameters such as component mass posteriors.
    \comment{I have a version of this plot with error bars, but they are so big that they are all totally consistent with each other.} 
    The two models differ most in their predictions for the number of events in the ranges $m_2\in [m_{\min}, 30\Msun]$ and $m_2\in [30\Msun,40\Msun]$ for all values of $m_1$ considered.
}
    \label{fig:PPCs}
\end{figure}

%%%% 
When validating astrophysical predictions of the properties of individual BHs, such as the outputs of single-star evolution codes, it is best to compare directly to $p_1(m_1)$ or $p_2(m_2)$, as defined in Equation~\ref{eq:pairing function} and shown in Figure~\ref{fig:bucket distributions}.
When examining properties of all lower mass BHs in a binary for all values of the higher mass BH, such as the outputs of population synthesis codes, it is appropriate to compare with the marginal secondary mass distribution as defined in Equation~\ref{eq:marginal m2}, and vice versa for the higher mass BH.
